Iterated Regret Minimization in Game Graphs

Iterated regret minimization has been introduced recently by J.Y. Halpern and R. Pass in classical strategic games. For many games of interest, this new solution concept provides solutions that are judged more reasonable than solutions offered by traditional game concepts -- such as Nash equilibrium --. Although computing iterated regret on explicit matrix game is conceptually and computationally easy, nothing is known about computing the iterated regret on games whose matrices are defined implicitly using game tree, game DAG or, more generally game graphs. In this paper, we investigate iterated regret minimization for infinite duration two-player quantitative non-zero sum games played on graphs. We consider reachability objectives that are not necessarily antagonist. Edges are weighted by integers -- one for each player --, and the payoffs are defined by the sum of the weights along the paths. Depending on the class of graphs, we give either polynomial or pseudo-polynomial time algorithms to compute a strategy that minimizes the regret for a fixed player. We finally give algorithms to compute the strategies of the two players that minimize the iterated regret for trees, and for graphs with strictly positive weights only.

==> algograph.tex <==
\Section{Algorithm on Graphs}

In a first step, we prove that strategies that do not pass twice by
the same position are sufficient to minimize the regret. Then in a
second section we abstract strategies by sets of paths. Finally we
give an algorithm that solves the regret minimization problem in
pseudo-polynomial ti


\SubSection{From strategies to paths}

We denote by $\lf_1(G)$ the set of winning loop-free strategies in $G$.
Given a path $\pi = s_0\dots s_n$ in $G$ such that $s_n\in\target$, we denote by $\comp^2_G(\pi)$ the set
of finite paths \textit{compatible} with $\pi$, the set of paths
$\pi'$ such that all common prefixes of $\pi$ and $\pi'$ that end by a
node own by Player 2 are followed by the same game position. Formally,
$\comp^2_G(\pi)$ is defined as the
set of paths $\pi' = s'_0s'_1\dots s'_m$ such that for all
$i\in\{0,\dots,m-1\}$, if $s'_i\in S_2$ and $s'_0\dots s'_i = s_0\dots s_i$, then
$s'_{i+1} = s_{i+1}$. We now prove that:

%%     We denote by $\lf_1(G)$ the set of winning loop-free strategies in $G$. 
%%     Given a loop-free path $\pi = s_0\dots s_n$ in $G$ such that $s_n\in\target$, we denote by $\comp_G(\pi)$ the set
%%     of paths \textit{compatible} with $\pi$, defined as the
%%     set of paths $\pi' = s'_0s'_1\dots s'_m$ such that for all
%%     $i\in\{0,\dots,m-1\}$, if $s'_i\in S_2$ and there exists
%%     $j\in\{0,\dots,n-1\}$ such that $s'_i = s_j$ ($j$ is unique since
%%     $\pi$ is loop-free), then $s'_{i+1} = s_{j+1}$. 
%%     We now prove that:


    \begin{lemma}\label{lem:compa}
      Given a game arena $G$, 
      $$
      \reg_G\ =\ \min\limits_{\lambda_1\in \lf_1(G)}
      \max\limits_{\lambda_2\in\Lambda_2(G)} [u(\lambda_1,\lambda_2) -
        \min\limits_{\pi'\in \comp^2_G(\outcometarget(\lambda_1,\lambda_2))} u(\pi')]
      $$
      with $\min \varnothing = +\infty$.
    \end{lemma}


    \begin{proof}
      If $\lf_1(G)=\varnothing$, then by Theorem \ref{th:loopfree}, $\reg(G)=+\infty = \min
      \varnothing$. Otherwise let $\lambda_1\in \lf_1(G)$.  We have to prove
      
      $$
      \reg(\lambda_1) = \max\limits_{\lambda_2\in\Lambda_2}
          [u(\lambda_1,\lambda_2) - \min\limits_{\pi'\in\comp^2_G(\outcometarget(\lambda_1,\lambda_2))} u(\pi')]
      $$
      
      \noindent Let $\lambda_2$ which maximizes $\reg(\lambda_1)$, and $\lambda_1^* = \argmin\ \br(\lambda_2)$.
      Let $\pi = \outcometarget(\lambda_1,\lambda_2)$. Since
      $\lambda_1$ is loop-free, $\pi$ is loop-free as
      well. The strategies $\lambda_1^*$ and $\lambda_2$ define a
      path $\pi''$ from the root to some node of the objective. Clearly
      $\pi''\in\comp^2_G(\pi)$, therefore
      $$
       \min\limits_{\pi'\in\comp^2_G(\outcometarget(\lambda_1,\lambda_2))}
      u(\pi')\leq u(\pi')$$

      and we get 
      $$
      \reg(\lambda_1) \leq
      \max\limits_{\lambda_2\in\Lambda_2} [u(\lambda_1,\lambda_2) -
        \min\limits_{\pi'\in\comp^2_G(\outcometarget(\lambda_1,\lambda_2))}
        u(\pi')]$$.
      

      
      Conversely, let $\lambda_2$ which maximizes $u(\lambda_1,\lambda_2) -
      \min\limits_{\pi'\in\comp^2_G(\outcometarget(\lambda_1,\lambda_2))}
      u(\pi')$, and
      $\pi'\in\comp^2_G(\outcometarget(\lambda_1,\lambda_2))$ which
      minimizes $u(\pi')$. Let $\pi =
      \outcometarget(\lambda_1,\lambda_2)$. %
%
%%       The path $\pi$ is
%%       loop-free, and we can assume that $\pi'$ is loop-free as
%%       well (otherwise we can remove the loops and get a path of
%%       smaller weight).
%
      Note that $u(\pi')$ only depends on $\pi$ and not on the whole strategy
      $\lambda_2$. Indeed, any strategy $\lambda_2'$ such that 
      $\outcometarget(\lambda_1,\lambda_2') =
      \outcometarget(\lambda_1,\lambda_2)$ is such that $u(\pi')$ is
      minimal. In particular, we can construct a strategy
      $\lambda_2'$ such that $u(\pi') = \br(\lambda_2')$. Let $\pi' =
      \alpha_0\dots\alpha_m$, then
      $\lambda_2'$ is defined by $\lambda_2'(\alpha_0\dots\alpha_i) =
      \alpha_{i+1}$ if $\alpha_i\in S_2$ ($i=0,\dots,m-1$), and any
      other value for other histories (the
      choice of these values is not important). Let $\lambda_1^*$ be
      the best reponse to $\lambda_2'$. By definition of $\lambda_2'$
      and since $\pi'\in\comp^2_G(\pi)$,
      $\outcometarget(\lambda_1^*,\lambda_2')\in \comp^2_G(\pi)$, so that
      $u(\outcometarget(\lambda_1^*,\lambda_2')) \geq u(\pi')$, since
      $u(\pi')$ is minimal. Moreover, there exists a strategy
      $\lambda_1'$ such that $\outcometarget(\lambda'_1,\lambda_2') =
      \pi'$ (easily defined by following the choices made along the
      path $\pi'$). Since $\lambda_1^*$ is the best response to $\lambda_2'$, we have 
      $u(\outcometarget(\lambda_1^*,\lambda_2'))\leq
      u(\outcometarget(\lambda_1',\lambda_2'))$,
      i.e. $u(\outcometarget(\lambda_1^*,\lambda_2'))\leq
      u(\pi')$. Therefore $u(\outcometarget(\lambda_1^*,\lambda_2')) =
      u(\pi')$ and we have defined a strategy $\lambda_2'$
      such that
      $$
      u(\lambda_1,\lambda_2) -
      \min\limits_{\pi'\in\comp^2_G(\outcometarget(\lambda_1,\lambda_2))}
      u(\pi') = u(\lambda_1,\lambda_2') - \br(\lambda_2')$$
      
      Since $\reg(\lambda_1)\geq u(\lambda_1,\lambda_2') -
      \br(\lambda_2')$, we get

      $$\reg(\lambda_1) \geq  u(\lambda_1,\lambda_2) -
      \min\limits_{\pi'\in\comp^2_G(\outcometarget(\lambda_1,\lambda_2))}
      u(\pi')$$.
\end{proof}

%%     We say that a weighted game arena  $G$ is \textit{pruned} if  Player 1 has a strategy to reach
%%     the objective from any node of the graph. It is possible to prune
%%     an arena in linear time by solving a reachability game. The regret
%%     of a \text{pruned} graph is always finite.
%%     We denote by $W_1(G)$ the set of \textbf{winning and loop-free} Player 1's strategies in $G$.
%%     Given a path $\pi = s_0\dots s_n$ in $G$ such that $s_n\in\target$, we denote by $\comp_G(\pi)$ the set
%%     of loop-free paths \textit{compatible} with $\pi$, defined as the
%%     set of paths $\pi' = s'_0s'_1\dots s'_m$ such that for all
%%     $i\in\{0,\dots,m-1\}$, if $s'_i\in S_2$ and there exists
%%     $j\in\{0,\dots,n-1\}$ such that $s'_i = s_j$, then $s'_{i+1} =
%%     s_{j+1}$.  

%%     We now prove that:


%%     \begin{lemma}\label{lem:compa}
%%       Given a pruned weighted game arena $G$, 
%%       $$
%%       \reg_G\ =\ \min\limits_{\lambda_1\in W_1(G)}
%%       \max\limits_{\lambda_2\in\Lambda_2(G)} [u(\lambda_1,\lambda_2) - \min\limits_{\pi'\in\comp_G(\outcometarget(\lambda_1,\lambda_2))} u(\pi')]
%%       $$
%%     \end{lemma}


%%     \begin{proof}
%%       By Theorem \ref{th:loopfree} and since $G$ is pruned, we have
%%       $\reg_G = \min\limits_{\lambda_1\in W_1(G)} \max\limits_{\lambda_2\in\Lambda_2(G)} [u(\lambda_1,\lambda_2)-\br(\lambda_2)]$.
%%       Therefore given $\lambda_1\in W_1(G)$,  we only have to prove
      
%%       $$
%%       \reg(\lambda_1) = \max\limits_{\lambda_2\in\Lambda_2} [u(\lambda_1,\lambda_2) - \min\limits_{\pi'\in\comp_G(\outcometarget(\lambda_1,\lambda_2))} u(\pi')]
%%       $$
      
%%       Let $\lambda_2$ which maximizes $\reg(\lambda_1)$, and $\lambda_1^* = \argmin\ \br(\lambda_2)$.
%%       Let $\pi = \outcometarget(\lambda_1,\lambda_2)$ (note that $\pi$
%%       is loop-free). We can assume that $\lambda_1^*$ is loop-free as well.
%%       The strategies $\lambda_1^*$ and $\lambda_2$ define a
%%       path $\pi'$ from the root to some node of the objective. Clearly, $\pi'$ is loop-free and
%%       $\pi'\in\comp_G(\pi)$, therefore
%%       $\min\limits_{\pi''\in\comp_G(\outcometarget(\lambda_1,\lambda_2))}
%%       u(\pi'')\leq u(\pi')$, and we get $\reg(\lambda_1) \leq
%%       \max\limits_{\lambda_2\in\Lambda_2} [u(\lambda_1,\lambda_2) -
%%         \min\limits_{\pi''\in\comp_G(\outcometarget(\lambda_1,\lambda_2))}
%%         u(\pi'')]$.
      

      
%%       Conversely, let $\lambda_2$ which maximizes $u(\lambda_1,\lambda_2) -
%%       \min\limits_{\pi'\in\comp_G(\outcometarget(\lambda_1,\lambda_2))}
%%       u(\pi')$, and
%%       $\pi'\in\comp_G(\outcometarget(\lambda_1,\lambda_2))$ which
%%       minimizes $u(\pi')$. Note that $u(\pi')$ only depends on the
%%       path $\outcometarget(\lambda_1,\lambda_2)$ and not on the whole strategy
%%       $\lambda_2$. Indeed, all strategy $\lambda_2'$ such that 
%%       $\outcometarget(\lambda_1,\lambda_2') =
%%       \outcometarget(\lambda_1,\lambda_2)$ are such that $u(\pi')$ is
%%       minimal. In particular, there is such a strategy $\lambda_2'$ such
%%       that $u(\pi') = \min_{\lambda_1^*\in\Lambda_1(G)}
%%       u(\lambda_1^*,\lambda_2')$. If $\pi' = \alpha_0\dots\alpha_m$
%%       and $\pi = \beta_0\dots\beta_n$, then
%%       $\lambda_2'$ is defined by $\lambda_2'(h\alpha_i) =
%%       \alpha_{i+1}$ if $\alpha_i\in S_2$, $\lambda_2'(h\beta_i) =
%%       \beta_{i+1}$ if $\beta_i\in S_2$, and any value otherwise (the
%%       choice of this value is not important). Let $\lambda_1^*$ be
%%       the best reponse to $\lambda_2'$. By definition of $\lambda_2'$,
%%       $\outcometarget(\lambda_1^*,\lambda_2')$ is necessarily
%%       compatible with $\outcometarget(\lambda_1,\lambda_2)$, so that
%%       $u(\outcometarget(\lambda_1^*,\lambda_2')) = u(\pi')$, since
%%       $u(\pi')$ is minimal. Therefore we have defined a strategy $\lambda_2'$
%%       such that $u(\lambda_1,\lambda_2) -
%%       \min\limits_{\pi'\in\comp_G(\outcometarget(\lambda_1,\lambda_2))}
%%       u(\pi') = u(\lambda_1,\lambda_2') - \min\limits_{\lambda_1^*}
%%       u(\lambda_1^*,\lambda_2')$, from which we get
%%       $\reg(\lambda_1) \geq  u(\lambda_1,\lambda_2) -
%%       \min\limits_{\pi'\in\comp_G(\outcometarget(\lambda_1,\lambda_2))}
%%       u(\pi')$.
%% \end{proof}


Let $G = (S = S_1\uplus S_2, s_0,T,\mu,\target)$ be a game arena with
target $\target$. For all path $\pi$ from $s_0$ to a target node, we
let $r(\pi)$ be the \textit{regret} of $\pi$, defined as

$$
r(\pi) = u_G(\pi) - \min\limits_{\pi'\in\comp^2_G(\pi)} u_G(\pi')
$$

The value $r(\pi)$ is
finite since $u_G(\pi)$ is finite and $\pi\in\comp^2_G(\pi)$. 
From Lemma \ref{lem:compa}, we know that:

$$
\reg_G\ =\ \min\limits_{\lambda_1\in \lf_1(G)}
\max\limits_{\lambda_2\in\Lambda_2(G)}
r(\outcometarget(\lambda_1,\lambda_2))\quad (\star)
$$

    

    For a given loop-free winning strategy $\lambda_1\in\lf_1(G)$ of Player 1, the aim of Player 2 is to choose a finite path
    $\pi$ reaching the target and ``compatible'' with $\lambda_1$ such
    that $r(\pi)$ is maximal.  Formally, the set of paths compatible
    with $\lambda_1\in\lf_1(G)$ is defined by:

    $$
    \comp_G^1(\lambda_1) = \{ s_0\dots s_n\ |\ s_n\in\target,\ \forall
    i< n, s_i\in S_1\implies s_{i+1} = \lambda_1(s_0\dots s_i)\}
    $$


%%     Note that for all
%%     $\pi\in\comp^1_G(\lambda_1)$, $\pi$ is loop-free. Then:

    \begin{proposition}\label{prop:minmax} $
    \reg_G = \min_{\lambda_1\in \lf_1(G)} \max_{\pi\in\comp^1_G(\lambda_1)} r(\pi)
    $
    \end{proposition}

    \begin{proof}
      Note that $r(\pi)$ is well-defined since $\pi$ necessarily
      reaches a target node, by definition of $\comp_G^1(\lambda_1)$.
      Let $\lambda_1\in\lf_1(G)$. Thanks to equation $(\star)$, we only
      have to prove that 
      $$
      \max\limits_{\lambda_2\in\Lambda_2(G)}
      r(\outcometarget(\lambda_1,\lambda_2)) =       
      \max_{\pi\in\comp^1_G(\lambda_1)} r(\pi)
      $$


      Let $\lambda_2\in \Lambda_2(G)$ that maximizes the expression on
      the left, and let $\pi =
      \outcometarget(\lambda_1,\lambda_2)$. We necessarily have
      $\pi\in\comp_G^1(\lambda_1)$. Therefore we get the inequality
      $\leq$. Conversely, let $\pi\in\comp_G^1(\lambda_1)$ that
      maximizes the expression on the right. We can define $\lambda_2$
      such that $\outcometarget(\lambda_1,\lambda_2)=\pi$ as follows:
      for all history $h$ and positions $v,v'$, $\lambda_2(hv) = v'$
      if $hvv'$ is a prefix of $\pi$ and $v\in S_2$, otherwise
      $\lambda_2(hv) = v'$ for some $v'$ (the chosen value is not
      important). By definition of $\lambda_2$,
      $\outcometarget(\lambda_1,\lambda_2) = \pi$, and therefore we
      get the inequality $\geq$. 
    \end{proof}


    From Proposition \ref{prop:minmax}, we can see that once Player 1
    has fixed a strategy $\lambda_1\in\lf_1(G)$ (if it exists), the
    regret of $\lambda_1$ does not depend on the strategies
    $\lambda_2$ that maximizes it, but only on the paths $\pi$
    compatible with $\lambda_1$ that maximize $r(\pi)$. Therefore,
    once $\lambda_1$ is fixed, the regret maximization problem (for
    Player 2) only deals with paths and not strategies. We now define
    the notion of best response to a path. For all position $v\in S_1\cup S_2$, we let

    $$
    \best(v) = \min\limits_{\lambda_1\in
      \Lambda_1(G,v)}\min\limits_{\lambda_2\in\Lambda_2(G,v)}
    u_G(\lambda_1,\lambda_2)
    $$

    For all path $\pi=s_0\dots s_n$ in $G$, we define the \textit{best
      alternative} to $\pi$ as follows:

    $$
    \ba(\pi)\ =\ \min_{i<n, s_i\in S_1, s\neq s_{i+1}, (s_i,s)\in T}
    u(s_0\dots s_i) + \mu(s_i,s) + \best(s)
    $$

    Finally, the \textit{best reponse} to $\pi$ is defined as follows:

    $$
    \br(\pi)\ =\ \min\ (u_G(\pi),\ \ba(\pi))
    $$


    Intuitively, when Player 1 chooses a winning strategy $\lambda_1$,
    and Player 2 chooses a path $\pi\in\comp_G^1(\lambda_1)$ that maximizes
    $r(\pi)$, the best alternative to $\pi$ is the best value
    different from $u_G(\pi)$ Player 1 could have achieved if he knew
    that Player 1 had chosen $\pi$. In other words, since $\pi$
    represents somehow a set of Player 2's strategies that maximize
    the regret, the best response to $\pi$ is the minimal best
    response to all those strategies. The next
    proposition states that the notions of regret of a path and best
    response to a path are related as in the usual definition of
    regret for strategies:


    \begin{proposition} \label{prop:rpi}
    For all $\lambda_1\in \lf_1(G)$, for all path $\pi\in\comp^1_G(\lambda_1)$,

    $$
    r(\pi) = u_G(\pi) - \br(\pi)
    $$

    with $\min\varnothing = +\infty$.
    \end{proposition}

    \begin{proof}
      We have to prove
      $$
      \min\limits_{\pi'\in\comp_G^2(\pi)} u_G(\pi') = \br(\pi)
      $$


      Let $\pi = s_0\dots s_n$. Let $\pi'$ that minimizes the expression on the left. If $\pi' =
      \pi$, then we get the inequality $\geq$. If $\pi' \neq \pi$,
      then let $s_0\dots s_i$ be the longest common prefix of $\pi'$ and
      $\pi$.  Then necessarily $s_i\in S_1$ by definition of
      $\comp_G^2(\pi)$. It is clear that $u_G(\pi') \geq u_G(s_0\dots s_is) + \best(s)$, for
      the position $s$ such that $s_0\dots s_is$ is a prefix of
      $\pi'$. Let $\pi''$ the path starting from $s$ that corresponds
      to $\best(s)$. We have $s_0\dots s_is\pi''\in\comp_G^2(\pi)$,
      and since $u_G(\pi')$ is minimal, we have $u_G(\pi') \geq
      u_G(s_0\dots s_is) + \best(s)$. Therefore we get the inequality
      $\geq$.

      
      Conversely, suppose that $u_G(\pi) = \br(\pi)$.
      Since $\pi\in\comp_G^2(\pi)$, we get the inequality
      $\leq$. Suppose that $u_G(s_0\dots s_is)+\best(s) = \br(\pi)$,
      , for some $s_i\in S_1$ and $s\neq
      s_{i+1}$ and $(s_i,s)\in T$. Let $\pi''$ the path starting from
      $s$ that corresponds to $\best(s)$. We have $s_0\dots
      s_is\pi''\in\comp_G^2(\pi)$, so that we also get the inequality $\leq$.
    \end{proof}




\SubSection{A pseudo polynomial-time algorithm}





In this section, we prove the regret minimization problem to be polynomial-time reducible
to a min-max game. We consider game graphs where weights are on the objective nodes -- called \textit{target-weighted game arena} --. Formally, the game graph with objective $\target$ 
is equipped with a weight function $\mu:\target\rightarrow \mathbb{N}$. The utility of a strategy $\lambda_1$ against a strategy $\lambda_2$ is
defined as $u(\lambda_1,\lambda_2) = +\infty$ if $\lambda_1$ is loosing, and $\mu(\last(\outcometarget(\lambda_1,\lambda_2)))$ otherwise.
The notions of best response and regret are defined accordingly to this utility function.
In particular, the regret of a loosing strategy is infinite. This problem can be seen as a particular case of the game graphs with weighted edges where all edge weights are $0$ except edges $(v,v')$ where $v'\in \target$ which are weighted by
$\mu(v')$ (if there is no incoming edge to some target node, this node is necessarily the starting node, and we can add a virtual edge that points to this node).








    Proposition \ref{prop:minmax} suggests that the regret
    minimization problem can be reduced to a minmax problem in a
    target-weighted arena $G'$ where the values $r(\pi)$ are attached to the
    target nodes, for all loop-free path $\pi$ of $G$ that ends up in
    a target node. In particular, 
    we construct a graph $G'$ such that any loop-free path $\pi$
    in $G$ that ends up in a target node corresponds to a loop-free path in $G'$
    ending up in a target node weighted by $r(\pi)$. And any
    loop-free path in $G'$ that ends up in a target node weighted by a
    value $e$ corresponds to a loop-free path $\pi$ in $G$ such that
    $r(\pi) = e$. To compute such a graph, one needs to compute the
    values $r(\pi)$ for all loop-free path $\pi$. One could enumerate 
    all loop-free path $\pi$ and compute its value $r(\pi)$, but it
    would result in an exponential time complexity. However
    Proposition \ref{prop:rpi} gives a way to compute all the values
    $r(\pi)$ by traversing the graph (and storing the weight of the
    current path and the best values seen along this path) , and whose complexity depends
    only polynomially on the size of the graph and the number of possible values
    $r(\pi)$ (which is polynomial in the graph arena and the maximal
    weight, as explained further). 

    
    
    We denote by $\mathbb{N}_k$ the set $\{0,1\dots,k\}$. 
    The graph $G'$ is constructed as follows.     


    \begin{definition}
      \label{def:Gprime}
      Let $G = (S = S_1\uplus S_2,s_0,T,\mu)$ a weighted graph arena
      with objective $\target$. Let $M = |\{ u(\pi)\ |\ \pi\text{ loop-free path in $G$ starting
      at $s_0$}\}|$. The target-weighted graph arena $G' =
      (S'_1,S'_2,T',s'_0,\mu')$ with objective $\target'$ associated
      with $G$  is defined
      as follows. The sets $S'_1,S'_2, T'$ are the least sets such
      that:    

    \begin{itemize}
        \item $S'_i\subseteq S_i\times \mathbb{N}_M \times
          (\mathbb{N}_M\cup\{+\infty\})$, $i=1,2$;
        \item $s'_0=(s_0,0,+\infty)\in S'_i$ if $s_0\in S_i$;
        \item $\forall (s,u,b)\!\!\in\!\! S'_1\!\cup\! S'_2,\ \forall
          i\in\{1,2\},\ \forall s'\in S_i,\ \forall u'\in
          \mathbb{N}_M,\ \forall b'\in \mathbb{N}_M\cup\{+\infty\}$,
          $((s,u,b),(s',u',b'))\in T'$ and $(s',u',b')\in
          S'_i$ if
          \begin{itemize}
          \item $(s,s')\in T$
          \item $u' = u+\mu(s,s')$ and $u'\leq M$
          \item $b'\leq M$ and $b' = \left\{\begin{array}{llll} \min (b,
            \min\limits_{(s,s'')\in T,s'\neq s''}
            u + \mu(s,s'')+\best(s'')) &\text{ if } s\in S_1 \\
          b & \text{ if } s\in S_2\end{array}\right.$
          \end{itemize}
    \end{itemize}

    The target and the weight function are defined by:

    \begin{itemize}
  
    \item $\target' = \{ (s,u,b)\in S'_1\cup S'_2\ |\ s\in \target\}$
    \item $\mu' : (s,u,b)\in\target' \mapsto u - \min (u, b)$
    
    \end{itemize}

    \end{definition}


From now on, we let $G = (S = S_1\uplus S_2,s_0,T,\mu)$ a game arena
with objective $\target$, and we let $G'$ be its associated
target-weighted game arena as in defined in the previous
definition. We let $S' = S'_1\cup S'_2$.
The values $\best(s)$ for all positions $s$ can be computed in
polynomial time, and $M \leq |S|\max_{(s,s')\in T} \mu(s,s')$. That
makes the construction of $G'$ doable in pseudo-polynomial time, as
stated by the next proposition:

\begin{proposition}\label{prop:complexity}
  The graph $G'$ can be computed in time complexity
  $O(|S||T|(M+2)^2)$. It has at most
    $|S|(M+2)^2$ vertices and $|T|(M+2)^2$ edges.
\end{proposition}


\begin{proof}
  Note that $|T'|\leq |T|(M+2)^2$. One can compute in $O(|S|(|S|+|T|))$ a
  data-structure that gives in constant time the value $\best(s)$,
    for all $s\in S$. For all $(s,u,b)\in
    S'$, and all $s'$ such that $(s,s')\in T$, computing $u',b'$ such
    that $((s,u,b),(s',u',b'))\in T'$ can be therefore done in 
    $O(|T|)$. It has at most $|S|(M+2)^2$ vertices, therefore it can
    be computed in time complexity $O(|S|(|S| + |T|) + |T||S|(M+2)^2) =
    O(|S||T|(M+2)^2+|S|^2) = O(|S||T|(M+2)^2)$.
\end{proof}


    We denote by $p_i(s,u,b)$ the $i$-th projection of a triple
    $(s,u,b)$. By extension, for a path $\pi$ in $G'$, $p_1(\pi)$ is
    word of first projections (note the it is also a path in $G$).

\begin{proposition}\label{prop:rr}
    Let $\pi = (s_0,u_0,b_0)\dots (s_n,u_n,b_n)$ be a finite path in
    $G'$ that starting in $s'_0 = (s_0,u_0,b_0)$ and such that 
    $(s_n,u_n,b_n)\in \target'$. Then:
    \begin{itemize}

    \item[$(i)$]  for all $i\leq n$, $u_i = u_G(s_0\dots s_i)$;
    
    \item[$(ii)$] for all $i\leq n$, $b_i = \ba(s_0\dots s_i)$;

    \item[$(iii)$] $u_{G'}(\pi) = r(p_1(\pi))$.
    
    \end{itemize}
\end{proposition}


\begin{proof}
  $(i)$ It is true at rank $0$, since by definition of $G'$, $u_0 =
  0 = u_G(s_0)$. Let $0<i<n$. If $u_i =u_G(s_0\dots s_i)$, then by
  definition of $G'$, $(s_i,s_{i+1})\in T$ and $u_{i+1} = u_i +
  \mu(s_i,s_{i+1}) = u_G(s_0\dots s_{i+1})$.

  


  $(ii)$ Clearly, it is true at rank $0$. Suppose that it is true at rank
  $i<n$. Suppose that $s_i\in S_2$, then by definition of $G'$,
  $b_{i+1} = b_i$ and we easily get the result since $\{
  j<i\ |\ s_j\in S_1\} = \{ j<i+1\ |\ s_j\in S_1\}$.
  Suppose that $s_i\in S_1$, then by definition of $G'$, 
  $b_{i+1} = \min (b_i, \min_{(s_i,s)\in T,s\neq s_{i+1}}
  u_i+\mu(s_i,s)+\best(s)$, i.e. $b_{i+1} = \min (b_i, \min_{(s_i,s),
    s\neq s_{i+1}} u_G(s_0\dots s_is) + \best(s)$, from which we get
  $b_{i+1} = \min \{ u_G(s_0\dots s_js)+\best(s)\ |\ j< i+1, s_j\in
  S_1,(s_j,s)\in T, s\neq s_{j+1}\}$.



  $(iii)$ By definition of $G'$, $u_{G'}(\pi) = u_n-\min(u_n,b_n) =
  u_G(p_1(\pi)) - \br(p_1(\pi))$ from $(i)$ and $(ii)$, i.e. $u_{G'}(\pi) =
  r(p_1(\pi))$, by Proposition \ref{prop:rpi}.
\end{proof}



A winning strategy $\lambda_1\in\Lambda_1(G')$ is said to
\textit{strongly loop-free} if for all $\lambda_2\in\Lambda_2(G')$,
$p_1(\outcometargetp(\lambda_1,\lambda_2))$ is loop-free.

\begin{proposition}\label{prop:stronglyloopfree}
  If there is a winning strategy for Player 1 in $G'$, 
  there is a Player 1's strongly loop-free strategy
  $\lambda_1\in\Lambda_1(G')$
  which minimizes $\max_{\lambda_2\in\Lambda_2(G')}
  u_{G'}(\lambda_1,\lambda_2)$.
\end{proposition}

\begin{proof}
  Let $\lambda_1$ which minimizes $\max_{\lambda_2\in\Lambda_2(G')}
  u_{G'}(\lambda_1,\lambda_2)$. This value is finite since
  there is winning strategy for Player 1 in $G'$, and therefore
  $\lambda_1$ is a winning strategy. Note that for all finite play
  $h$ such that $\last(h)\in S'_1$, $\lambda_1(h)$ only depends on
  $p_1(h)$, since $p_2(h)$ and $p_3(h)$ are uniquely determined by
  $p_1(h)$, by definition of $G'$. Therefore we assume wlog in the
  sequel that Player 1's strategies are mappings from $(S_1\cup S_2)^*S_1$ to $S'_1\cup
  S'_2$. Suppose that $\lambda_1$ is not
  strongly loop-free. Therefore there exists a strategy 
  $\lambda_2\in\Lambda_2(G')$ such that $\pi =
  \outcometargetp(\lambda_1,\lambda_2)$ is not strongly loop-free.
  Let $\pi = (s_0,u_0,b_0)\dots (s_n,u_n,b_n)$. There exist
  $0\leq i<j\leq n$ such that $s_i = s_j$. We let $\lambda'_1$ a
  Player 1's strategy in $G'$ defined as follows: for all finite play
  $h$ such $\last(h)\in S_1$, 

  $$
  \lambda'_1(h) = \left\{\begin{array}{llllll}
  \lambda_1(s_0\dots s_i\dots s_jh') & \text {if } h = s_0\dots
  s_ih'\text{ for some $h'$} \\
  \lambda'_1(h) & \text{otherwise } 
    \end{array}\right.
  $$

  We now prove that 

  $$
  \max_{\lambda_2\in\Lambda_2(G')}
  u_{G'}(\lambda_1,\lambda_2) =   \max_{\lambda_2\in\Lambda_2(G')}
  u_{G'}(\lambda'_1,\lambda_2)
  $$

  We only have to prove the inequality $\geq$ by minimality of
  $\lambda_1$. Let $\lambda'_2$ which maximizes
  $u_{G'}(\lambda'_1,\lambda'_2)$. Let $\pi' =
  \outcometargetp(\lambda'_1,\lambda'_2)$. If $s_0\dots s_i$ is not a
  prefix of $\pi'$, then $\outcometargetp(\lambda_1,\lambda'_2) =
  \pi'$, and therefore $u_{G'}(\lambda_1,\lambda'_2) =
  u_{G'}(\lambda'_1,\lambda'_2)\leq \max_{\lambda_2\in\Lambda_2(G')}
  u_{G'}(\lambda_1,\lambda'_2)$. If $\pi' = s_0\dots s_i\pi''$ for some
  $\pi''$, then can construct a strategy $\lambda_2$ such that
  $u_{G'}(\lambda'_1,\lambda'_2)\leq u_{G'}(\lambda_1,\lambda_2)$. The
  strategy $\lambda_2$ is defined as follows:

  $$
  \lambda_2(h) = \left\{\begin{array}{llllll}
%%   \lambda'_2(h) & \text{if $h$ is a strict prefix of } s_0\dots s_i \\
  s_{k+1} & \text{if } h = s_0\dots s_i\dots s_k \text{ where } i\leq k<j \\
  \lambda'_2(s_0\dots s_ih') & \text {if } h = s_0\dots s_i\dots s_jh'\text{ for some $h'$} \\
  \lambda'_2(h) & \text{otherwise } 
    \end{array}\right.
  $$
  

  By definition of $\lambda_2$, we have
  $\pi_1 := \outcometargetp(\lambda_1,\lambda_2) = s_0\dots s_i\dots s_jh$ and
  $\outcometargetp(\lambda'_1,\lambda'_2) = s_0\dots s_ih$, for some
  $h$. Therefore $u_G(\pi') \leq u_G(\pi_1)$, and $\ba(\pi')\geq
  \ba(\pi_1)$. It is not difficult to verify that it implies
  $r(\pi')\leq r(\pi_1)$, i.e. $u_{G'}(\pi')\leq u_{G'}(\pi_1)$.
  Therefore

  $$
  u_{G'}(\pi') = \max_{\lambda_2\in\Lambda_2(G')}
  u_{G'}(\lambda'_1,\lambda_2) \leq u_{G'}(\pi_1)\leq   \max_{\lambda_2\in\Lambda_2(G')}
  u_{G'}(\lambda_1,\lambda_2)
  $$

  Finally, by an argument similar to the construction of $\lambda_2$,
  it is easy to show that $\sum_{\pi\in\{
  \outcometargetp(\lambda'_1,\lambda_2)\ |\ \lambda_2\in\Lambda_2(G')\}}
  |\pi| < \sum_{\pi\in\{
  \outcometargetp(\lambda_1,\lambda_2)\ |\ \lambda_2\in\Lambda_2(G')\}}
  |\pi|$. Therefore, we can iterate the previous construction (from
  $\lambda_1$ to $\lambda'_1$) until we get a loop-free strategy whose
  value is the same as $\lambda_1$.
 \end{proof}



We now prove that the reduction to a minmax game is correct:

\begin{proposition}\label{prop:correctness}
    $$ \reg(G) = 
     \min_{\lambda_1\in\Lambda_1(G')}
    \max_{\lambda_2\in\Lambda_2(G')} u_{G'}(\lambda_1,\lambda_2)$$
\end{proposition}

\begin{proof}
Let $\minmax(G') = \min_{\lambda_1\in\Lambda_1(G')} \max_{\lambda_2\in\Lambda_2(G')} u(\lambda_1,\lambda_2)$.


    \begin{itemize}
      \item $\reg(G)\geq \minmax(G')$. If $\reg(G) = +\infty$, the
        property obviously holds. Suppose that $\reg(G)< +\infty$ and
        let $\lambda_1\in\lf_1(G)$ which
        minimizes $\max\limits_{\pi\in\comp^1_G(\lambda_1)} r(\pi)$. We define
        $\tilde{\lambda_1}$ a strategy in $G'$ as follows:

        $$
        \tilde{\lambda_1}(h.(s,u,b)) = (\lambda_1(p_1(h).s), u',b')
        \text{ such that } ((s,u,b),(\lambda_1(p_1(h).s), u',b'))\in T'
        $$

        It is well-defined as for all $s'$ such that $(s,s')\in T$,
        there exists exactly one $u'$ and one $b'$ such that
        $((s,u,b),(s',u',b'))\in T'$, by definition of $G'$.
        Since $\lambda_1$ is winning in $G$, $\tilde{\lambda_1}$ is
        also winning in $G'$. Let $\pi\in\comp^1_G(\lambda_1)$  such that
        $r(\pi)$ is maximal. Since $\lambda_1$ is loop-free,  $\pi$ is
        loop-free.  We define a strategy $\tilde{\lambda_2}\in
        \Lambda_2(G')$ such that
        $u(\tilde{\lambda_1},\tilde{\lambda_2}) = r(\pi)$ and
        $\tilde{\lambda_2}$ is
        maximal -- i.e. for all $\lambda_2'$,
        $u(\tilde{\lambda_1},\lambda_2')\leq
        u(\tilde{\lambda_1},\tilde{\lambda_2})$--.
        Let $\pi = s_0s_1\dots s_n$. 

        $$
        \tilde{\lambda_2}(h(s,u,b)) = \left\{\begin{array}{llll}
        (s_{i+1},u',b') & \text{ if } \exists i, s_i = s\text{ and }
        ((s,u,b),(s_{i+1},u',b'))\in T' \\

        (s',u',b') & \text{ for some $(s',u',b')$ s.t. }
        ((s,u,b),(s',u',b'))\in T'   \text{ otherwise}\\
        
        \end{array}\right.
        $$


        By definition of $\tilde{\lambda_1}$ and $\tilde{\lambda_2}$,
        $\outcometarget_{G}(\lambda_1,\lambda_2) =
        p_1(\outcometarget_{G'}(\tilde{\lambda_1},\tilde{\lambda_2}) =
        \pi$,
        and therefore $u_{G'}(\tilde{\lambda_1},\tilde{\lambda_2}) =
        r(\pi)$. Suppose that it is not maximal. Therefore there
        exists $\tilde{\lambda_2}'$ such that
        $u_{G'}(\tilde{\lambda_1},\tilde{\lambda_2}') >
        u_{G'}(\tilde{\lambda_1},\tilde{\lambda_2})$. We let $\pi' =
        \outcometarget(\tilde{\lambda_1},\tilde{\lambda_2}')$.
        We prove that $p_1(\pi')\in\comp^1_G(\lambda_1)$ and
        $r(p_1(\pi'))>r(\pi)$, which is a contradiction.
        Let $\pi' = (v_0,u_0,b_0)\dots (v_m,u_m,b_m)$. 
        By definition of $\tilde{\lambda_1}$, for all
        $i\in\{0,\dots,m-1\}$, if $v_i\in S_1$, then $v_{i+1} =
        \lambda_1(v_0\dots v_m)$, and therefore $p_1(\pi')\in
        \comp^1_G(\lambda_1)$. Since $u_{G'}(\pi') = r(p_1(\pi'))$, we
        get $r(p_1(\pi'))>r(\pi)$, which is a contradiction. Therefore
        $\reg(G) \geq \minmax(G')$.


        \item $\reg(G)\leq \minmax(G')$. Wlog, suppose that $\minmax(G')<+\infty$.
          Let $\tilde{\lambda_1}$ a Player 1's strategy in $G'$ which minimizes
          $\max_{\tilde{\lambda_2}}
          u(\tilde{\lambda_1},\tilde{\lambda_2})$. By Proposition
          \ref{prop:stronglyloopfree}, we can assume $\tilde{\lambda_1}$ to be strongly
            loop-free.  We define $\lambda_1$ a Player 1's strategy in
          $G$ as follows:

          $$
          \lambda_1(h) = 
          p_1(\tilde{\lambda_1}(\last(h), u_G(h), \ba(h)))
          $$


          Note that $h$ is well-defined (i.e. is a finite play in
          $G'$). Since $\tilde{\lambda_1}$ is strongly loop-free and
          winning in $G'$, $\lambda_1$ is loop-free and winning in
          $G$.
          


          Let $\tilde{\lambda_2}$ which maximizes
          $u(\tilde{\lambda_1},\tilde{\lambda_2})$ and let $\pi =
          \outcometargetp_{G'}(\tilde{\lambda_1},\tilde{\lambda_2})$.
          Note that $\pi$ is strongly loop-free, and by definition of
          $\lambda_1$, $p_1(\pi)\in\comp^1_G(\lambda_1)$. We prove that
          $r(p_1(\pi))$ is maximal. Suppose that there exists $h =
          s_0s_1\dots s_n\in\comp^1_G(\lambda_1)$ such that $r(h) >
          r(p_1(\pi))$. We can define a strategy $\tilde{\lambda_2}'$
          such that
          $u(\tilde{\lambda_1},\tilde{\lambda_2}')>u(\tilde{\lambda_1},\tilde{\lambda_2})$,
          which is a contradiction. We let 


          $$
          \tilde{\lambda_2}'(h(s,u,b)) = \left\{\begin{array}{llll}
          (s_{i+1},u',b') & \text{ if } \exists i, s_i = s\text{ and }
          ((s,u,b),(s_{i+1},u',b'))\in T' \\
          
          (s',u',b') & \text{ for some $(s',u',b')$ s.t. }
          ((s,u,b),(s',u',b'))\in T'   \text{ otherwise}\\
          
          \end{array}\right.
          $$
          

          By definition of $\tilde{\lambda_2}'$, $h =
          p_1(\outcometargetp(\tilde{\lambda_1},\tilde{\lambda_2}'))$,
          and therefore
          $u_{G'}(\outcometarget(\tilde{\lambda_1},\tilde{\lambda_2}')
          = r(h) > r(p_1(\pi)) =
          u_{G'}(\outcometarget_{G'}(\tilde{\lambda_1},\tilde{\lambda_2}))$,
          which is a contradiction.
          Therefore $\reg(G)\leq \minmax(G')$.
    \end{itemize}

\end{proof}


\textbf{Remark:} A winning strategy $\tilde{\lambda_1}$ that minimizes
$\minmax(G')$ gives a strategy $\lambda_1$ in $G$ that minimizes the
regret. This strategy is defined by:

          $$
          \lambda_1(h) = 
          p_1(\tilde{\lambda_1}(\last(h), u(h), \ba(h)))
          $$

Therefore $\lambda_1$ is a finite-state strategy and the memory needed
is $S_1\times \mathbb{N}_M\times \mathbb{N}_M\cup \{+\infty\}$,
i.e. the last position, the utility of the path traversed so far (up
to $M$), and the best alternative along this path.


Conversely, any winning strategy $\lambda_1$ that minimizes the regret
in $G$ gives a strategy $\tilde{\lambda_1}$ in $G'$ that minimizes
$\minmax(G')$. It is defined by:


          $$
          \tilde{\lambda_1}(h) = (\lambda_1(p_1(h)),u,b)  \text{ where
          } (\last(h), (\lambda_1(p_1(h)),u,b))\in T'
          $$




From Propositions \ref{prop:complexity} and \ref{prop:correctness}, we
can now state the following theorem:


\begin{theorem}\label{th:reduction}
    Let $G = (S = S_1\uplus S_2,
    s_0,T,\mu)$ be a game arena with objective $\target$, and let $M = |\{ u(\pi)\ |\ \pi\text{ loop-free
      path in } G \text{ that starts in $s_0$}\}$.
    One can construct in time $O(|T||S|(M+2)^2)$ a
    target-weighted arena $G' = (S',s'_0,T',\mu')$ with objective $\target'$ such
    that:

    \begin{enumerate}
    \item $|S'| \leq |S|(M+2)^2$ and $|T'| \leq |T|(M+2)^2$
    \item for all $v'\in\target'$,
      $\mu'(v')\leq |S|\max_{(s,s')\in T}\mu(s,s')$ or
      $\mu'(v')=+\infty$

    \item $\reg(G)\ =\ \min\limits_{\lambda_1\in\Lambda_1(G')}
      \max\limits_{\lambda_2\in\Lambda_2(G')}
      u_{G'}(\lambda_1,\lambda_2)$
    \end{enumerate}
\end{theorem}


Finally, it allows us to solve the regret minimization problem:


\begin{theorem}\label{th:regretmin}
  Given a weighted game arena $G = (S = S_1\uplus S_2,
    s_0,T,\mu,\target)$, computing the regret for Player 1 in $G$ can
    be done in time $O(|S||T|(M+2)^4)$, where $M = |\{u(\pi)\ |\ \pi\text{ loop-free
      path in } G \text{ that starts in $s_0$}\}$.
\end{theorem}


\begin{proof}
  From Theorem \ref{th:reduction}, minimizing the regret amounts to
  solve a $\minmax$ game in a graph $G' = (S',T',s'_0,\mu',\target')$ as constructed in the proof
  of Theorem \ref{th:reduction}. Solving a min-max game can be done by
  a fixpoint algorithm in
  time $O(|S'|(|S'|+|T'|))$.Therefore the
  overall complexity of minimizing the regret is 

  $O(|T||S|(M+2)^2 + |S|(M+2)^2(|S|(M+2)^2 + |T|(M+2)^2)) =
  O((|S|^2(M+2)^4 + |S||T|(M+2)^4) = O(|S||T|(M+2)^4)$.
\end{proof}


\paragraph{Polynomial-time algorithm on target-weithed arenas} The
previous algorithm is in PTIME on target-weighted graph arenas, since
in this case $M \leq |\target| \leq |S|$. Therefore the regret
minimization problem can be solve in time $O(|S|^5|T|)$ on
target-weighted arenas.





==> algotree.tex <==
\Section{Iterated Regret on Trees}

We now consider that \emph{both} players have a set of objective
states. So, each leaf is labelled by two weights, one for each
player. We can compute regrets for both players with two independant
executions of the algorithm we defined above.

We consider only sets of strategies that can be represented by a tree. Let $T = \tuple{S = S_1\uplus S_2, s_0, E,c_1,c_2}$ be a tree. $\Lambda_1(T) $ (resp.  $\Lambda_2(T) $) is a set of strategies for
Player 1 (resp. Player 2) defined as:

\begin{itemize}
\item $\lambda_1\in \Lambda_1(T)$ if and only if $\forall s_1\in S_1 : (s_1,\lambda_1(s_1))\in E$ when $s_1$ is not a leaf
\item $\lambda_2\in \Lambda_2(T)$ if and only if $\forall s_2\in S_2 : (s_2,\lambda_2(s_2))\in E$ when $s_2$ is not a leaf
\end{itemize}


Note that when we add a {\it best alternative} function ($b_i: S\to
\mathbb{N}\cup\{+\infty\}$) to this tree, it does not change the
definition of $\Lambda_1(T) $ and $\Lambda_2(T)$.

We remind that $b_1$ is defined as:
\begin{itemize}
\item $b_1(s_0)= +\infty$
\item if $(s,s')\in E$ and $s \in S_1$, then $b_1(s')= \min\left(b_1(s),\min_{(s,s'')\in E, s''\neq s'} \best(s'')\right)$
\item if $(s,s')\in E$ and $s \in S_2$, then $b_1(s')=b_1(s)$
\end{itemize}
and $b_2$ is defined symetrically.

With this function, we can prove that for any strategy $\lambda_1 \in \Lambda_1(T)$ we have
$\reg_1(\lambda_1) = \reg_1(\lambda_1,T,b_1)$ where $ \reg_1(\lambda_1,T,b_1)$ is defined recursively as:
\begin{itemize}
\item $c_1(s)- \min(c_1(s),b_1(s))$ if $T$ is a leaf
\item $ \reg_1(\lambda_1^{/T'},T',b_1)$ if the root $s$ of $T$ belongs to $S_1$ and that $\lambda_1(s)= s'$ which is the root of $T'$
\item $\max_{T'} \reg_1(\lambda_1^{/T'},T',b_1) $  if the root $s$ of $T$ belongs to $S_2$
\end{itemize}


We define a 'delete' operator $D_1(T,k_1)$ that returns a subtree representing the strategies $\lambda_1\in \Lambda_1(T)$ such that $\reg_1(\lambda_1)\leq k_1$. 

\begin{definition}
  Let $T = (S = S_1\uplus S_2, s_0, E,c_1,c_2)$ be a weighted tree and $k_1 \geq 0$ be an integer. $D_1(T,k_1)$ is the subtree defined as:
 $$
    D_1(T,k_1)\ =\ \left\{\begin{array}{llllllll}
        \mathrm{empty tree}  & \text{ if } \reg_1(T)> k_1\\
    s_0\left(D(T_{i_1}),\dots,D(T_{i_m})\right) & \text{ if
    } T= s_0(T_1,\dots T_n)\text{ and } s_0\in S_1 \text{ and for all subtrees }T_i \text{ such that }  \reg_1(T_i)\leq k_1\\
    s_0\left(D(T_{1}),\dots,D(T_{n})\right) & \text{ if } T= s_0(T_1,\dots T_n)
    \text{ and } s_0\in S_2 \text{ and for all subtrees }T_i :  \reg_1(T_i)\leq k_1\\
     & \text{ if } T \text{ is a leaf and } \reg_1(T) \leq k_1
    \end{array}\right.
  $$

\end{definition}
We define $D_2(T,k_2)$ symetrically.


\begin{proposition}
\label{prop:deletion}
   Let $T = (S = S_1\uplus S_2, s_0, E,c_1,c_2)$ be a weighted tree, $\lambda_1\in \Lambda_1(T)$ and $k_1 \geq 0$.  $\reg_1(\lambda_1)\leq k_1$ if an only if $\lambda_1\in \Lambda_1(D_1(T,k_1))$.
\end{proposition}
A similar proposition holds for $D_2(T,k_2)$.

\begin{proof}
We prove that if $\lambda_1$ is a strategy allowed in $D_1(T,k_1)$, then $\reg_1(\lambda)\leq k_1$ by induction on the size of $T$.

If $T$ consists in a single leaf, then $\lambda_1 \in \Lambda_1(T)\implies  \reg_1(T) = reg_1(\lambda_1^{/T},T,b)\leq k_1 $

We assume that the property is true for any tree of a size lesser or
equal than $x$. We now consider a tree $T$ of size $x+1$.

If  $\lambda_1 \in \Lambda_1(T)$

If the root of $T$, $s$, belongs to $S_1$, then since $\lambda_1 \in \Lambda_1(D_1(T,k_1))$ means that $(s,\lambda_1(s))$ is an edge of $D_1(T,k_1)$ and that $\lambda_1^{/T'}$ is allowed in $T'$, the subtree rooted at $\lambda_1(s)$. By induction hypothesis, $\reg(\lambda_1^{/T'},T',b)\leq k_1$ thus  $\reg(\lambda_1,T,b)\leq k_1$.

If $s\in S_2$, then $\lambda_1 \in \Lambda_1(D_1(T,k_1))$ implies that $\lambda_1^{/T'}$ is allowed in any subtrees $T'$ of $D_1(T,k_1)$. by induction hypothesis on each subtrees, we have that  $\reg(\lambda_1^{/T'},T',b)\leq k_1$ for each subtree, thus $\reg(\lambda_1,T,b)\leq k_1$.


  To complete the proof, we do another induction on the size of $T$.
If $T$ consists in a single leaf, then $\reg_1(\lambda_1)\leq k_1 \implies  \reg_1(T)\leq k_1 \implies$ $\lambda_1$ is a strategy allowed in $D_1(T,k_1)$.

We assume that the property is true for any tree of a size lesser or
equal than $x$. We now consider a tree $T$ of size $x+1$.

If the root of $T$, $s$, belongs to $S_1$, then since $\reg_1(\lambda_1,T,b)=\reg_1(\lambda_1^{/T'},T',b)\leq k_1 \implies  \reg_1(T',b)\leq k_1$ where $T'$ is the subtree rooted at $\lambda_1(s)$. By induction hypothesis, $\lambda_1$ is allowed in  $D_1(T',k_1)$, so it is allowed in $D_1(T,k_1)$.

If $ s\in S_2$, then since $\reg_1(\lambda_1,T,b)\geq \reg_1(\lambda_1,T',b)$ for any subtree $T'$, we have $\reg_1(T')\leq k_1$. By induction hypothesis, $\lambda_1$ is allowed in  $D_1(T',k_1)$, so it is allowed in $D_1(T,k_1)$.

\end{proof}




We can now define a 'delete' operation $D(T)$ combining the two operations

\begin{proposition}
  $T = (S = S_1\uplus S_2, s_0, E,c_1,c_2)$ be a weighted tree. Let $k_1=\reg_1(T)$ and $k_2=\reg_2(T)$.
  Then $D_1(D_2(T,k_2),k_1)= D_2(D_1(T,k_1),k_2) = D(T)$
\end{proposition}

\begin{proof}
  We simply remark that for any $k_1,k_2$, $\lambda_1 \in \Lambda_1(T) \implies \lambda_1 \in \Lambda_1(D_2(T,k_2))$ and $\lambda_2 \in \Lambda_2(T) \implies \lambda_2 \in \Lambda_2(D_1(T,k_1))$
\end{proof}

According to Proposition \ref{prop:deletion}, $D(T)$
only keeps strategies minimizing the regrets. Its complexity is linear
w.r.t. the size of the tree assuming we computed the regrets and
stored their values. We can iterate it until stabilization.


==> dag.tex <==
\subsection{Iterated Regret Minimization in target-weighted \DAG arenas}

In this section, we let $i\in\{1,2\}$ and $G = (S=S_1\uplus
S_2,s_0,T,\mu^G_1,\mu^G_2,\target_1,\target_2)$ be an acyclic \twa. In
order to compute efficiently the iterated regret, we need a compact
representation of the subsets of strategies $P^j_i$.% ; we will
% demonstrate that $P^j_i$ can be represented by an acyclic \twa $H^j$,
% with $\Lambda_i(H_j)= P^j_i$.

In Section~\ref{sec:targetgraph}, we defined a \twa $G'$~(see
Definition~\ref{def:reduc})such that there are two bijective mappings
$\Phi_i: \Lambda_i(G) \to \Lambda_i(G')$ and that $\reg^{G,1}_i =
\reg^{G'}_i$. We will use a similar construction. Assuming that
$P^j_i$ can be given by an acyclic \twa $H^j$, with $\Lambda_i(H_j)=
P^j_i$, we will construct $G'$ such that there are two bijective
mappings $\Phi_i: P^j_i \to \Lambda_i(G')$ and that $\reg^{G,j}_i =
\reg^{G'}_i$. Moreover, when applying a delete operator on $G'$, we
obtain a \twa representation of the sets of strategies $P^{j+1}_i$.


In the following, $H$ is a \twa representing the two sets of strategies
$P_1$ and $P_2$. We assume that $H = (S^H = S^H_1 \uplus
S^H_2,s^H_0,T^H,\mu^{H}_1,\mu^{H}_2,\target^H_1,\target^H_2)$ with ~:
\begin{enumerate}
\item $S^H_i = S_i \times (\mathbb{N}_{w_m} \cup \{+\infty\})^2\times
  \{\true,\false\}^2 $
\item $s^H_0= (s_0,+\infty,+\infty, s_0\in\target_1,s_0\in\target_2)$
\item if $\left((s,b_1,b_2,o_1,o_2),(s',b'_1,b'_2,o'_1,o'_2) \right)
  \in T^H $ then $(s,s') \in T$
\item  $\target^H_i = \target_i \times (\mathbb{N}_{w_m})^2\times
  \{\true,\false\}^2 $
\item there are two injective mappings $\Phi_{H,i}^{-1}: \Lambda_i(H)
  \rightarrow \Lambda_i(G)$.
\end{enumerate}
In a state $(s,b_1,b_2,o_1,o_2)$, $b_1$ and $b_2$ represent the best
alternatives for Player 1 and 2. The boolean values $o_i$ are true if
the objective $\target_i$ has beed already reached. We need those two
values because when the objective $\target_i$ is reached, whatever
Player $i$ plays, it has no influence on her regret. When we compute
regret for both playr, we need this information because the
computation stops when both objectives are reached.
% Since our aim is
% to apply a operator deleting some edges to obtain the
% strategies minimizing the regret, we should not delete any edge when
% $\target_i$ is reached.


We redefine the notion of best alternative to an edge of $G$, when we
are restrict to the strategies of $P_1$ and $P_2$. We let~:
$$
\best^{G,P_i,P_{\m i}}_i(s) = \min_{\lambda_i\in P_i \cap \Lambda_i(G,s)}
\min_{\lambda_{\m i}\in P_{\m i} \cap \Lambda_{\m i}(G,s))} \ut^G_i(\lambda_i,\lambda_{\m i})
$$
and~:

$$
\ba^{G,P_i,P_{\m i}}_i(s,s') = \left\{\begin{array}{lllll}
+\infty & \text{ if } s\in S_{\m i} \\
\min_{(s,s'')\in T,s''\neq s'} \best^{G,P_i,P_{\m i}}_i(s) & \text{ if } s\in S_{i} \\
\end{array}\right.
$$

% Notice that when the objective $\target_i$ is reached, whatever Player
% $i$ plays, it has no influence on her regret. This is the reason why
% we should remember when an objective is reached. We add this
% information to the graph of best alternatives $G'$, where the best
% alternatives are computed according to a set of strategies given by
% $H$, and two boolean values storing whether an objective is
% reached. The construction is similar to the one of
% Section~\ref{sec:targetgraph}, but we restrict ourselves to the
% strategies allowed by $H$. We introduce a mapping $\Psi$ that help us
% to define what are the actions allowed by $H$.

% If $H=H_j$, then when applying a delete operator $D$ to $G'$,
% we will obtain $H_{j+1}$. 

\begin{definition}\label{def:reduc:iterated}
  Given $G= (S=S_1\uplus
  S_2,s_0,T,\mu^G_1,\mu^G_2,\target_1,\target_2)$ and $H= (S^H = S^H_1
  \uplus
  S^H_2,s^H_0,T^H,\mu^{H}_1,\mu^{H}_2,\target^H_1,\target^H_2)$, we
  let $P_i= \Phi_h^{-1}(\Lambda_i(H))$. We construct the graph of best
  alternatives $G' = (S'= S'_1 \uplus
  S'_2,s_0',T',\mu^{G'}_1,\mu^{G'}_1,\target'_1,\target'_2)$ and a
  relation $\Psi \subseteq S^H \times S'$ as the least set such as~:

\begin{itemize}
\item $S'_i = S_i \times (\mathbb{N}_{w_m} \cup \{+\infty\})^2\times \{\true,\false\}^2 $, $i=1,2$;
\item $s_0' = (s_0,+\infty,+\infty, s_0\in\target_1,  s_0\in\target_2 )$ and $(s^H_0, s'_0)\in\Psi$;
\item for all $h\in S^H$, for all $(s,b_1,b_2,o_1,o_2)\in S'$, for all
  $h'=(s',\beta_1,\beta_2,o'_1,o'_2)\in S^H$ such that $(h,h)\in T^H$,
  we have~: $\left(h, (s,b_1,b_2,o_1,o_2)\right)\in \Psi$ if and only if
  \begin{enumerate}
  \item $(s',b'_1,b'_2,o_1',o_2')\in S'$
  \item $\left(h',(s',b'_1,b'_2,o_1',o_2')\right)\in\Psi$
  \item $\left((s,b_1,b_2,o_1,o_2),(s',b'_1,b'_2,o'_1,o'_2)\right)\in T'$, where:
 \[
 \begin{array}{lcl}
   b'_i &=& \left\{\begin{array}{llll} \min (b_i,\ba_i^{G,P_i,P_{\m i}}(s,s')) &\text{ if } s\in S_i \\
       b_i & \text{ if } s\in S_{\m i}\end{array}\right.
 %   \\
%    o'_i &=& o_i \vee (s'\in\target_i)
 \end{array}
 \]
  \end{enumerate}
\end{itemize}

\end{definition}

To understand the difference between $H$ and $G'$, and the role of the
relation $\Psi$, we precise that at a step of the iterated fixpoint
computation, $H$ represents the two sets of strategies $P^j_1$ and
$P^j_2$. A state $h=(s,\beta_1,\beta_2,o_1,o_2)\in S^H$ is such that
$\beta_i= \best^{G,P_i^{j-1},P_{\m i}^{j-1} }_i$. A state
$s'=(s,b_1,b_2,o_1,o_2)\in S'$ is such that $b_i=
\best^{G,P_i^{j},P_{\m i}^{j} }_i$. $G'$ is intuitively the \twa $H$
where the best alternatives have been updated to match the values
$\ba^{G,P_i^{j},P_{\m i}^{j}}_i(s,s')$. However, there is no
one-to-one mapping between the two graphs, because two states $h_1$ and
$h_2$ that were leading to the same state $h_3$ of $S^H$ may now have
a different best alternative.  This is why we use the relation $\Psi$
in Definition~\ref{def:reduc:iterated}.


\begin{proposition}\label{lem:maxmax:iterated}
%   Let $i\in\{1,2\}$. For all $\lambda_i\in\Lambda_i(G')$,
%   $\reg^{G'}_i(\lambda_i)\! =\!\!\!\!\! \max\limits_{\lambda_{\m i}\in\Lambda_{\m i}(G')}
%   \nu_i(\lambda_1,\lambda_2)$}.

% Moreover~:
Let $i\in\{1,2\}$, and $G'$, $P_i$ $P_{\m i}$ defined as in Definition~\ref{def:reduc:iterated}~:
\vspace{-2mm}
  $$
  \reg^{G,P_i,P_{\m i}}_i = \minmax^{G'}_i
  $$

\vspace{-3mm}
\end{proposition}


In order to prove this proposition, we define a bijective mapping
$\Phi_i\;:\; \Lambda_{i}(H) \rightarrow \Lambda_{i}(G')$. Let $i\in\{1,2\}$ and
$\lambda_i\in\Lambda_i(H)$.  Let $\pi\in\play_f(G')$ such that
$\last(\pi)=(s,b_1,b_2,o_1,o_2)\in S'_i$ and let $p_1(h)\in S^*$ be the
sequence of first projections of elements of $h$.  Let $s' =
\lambda_i(p_1(h))$.  Then $\Phi(\lambda_i)(h) =
(s',b'_1,b'_2,o'_1,o'_2)$ where, $b'_i$ and $o'_i$ are defined in the
same way as the transition function of
Definition~\ref{def:reduc:iterated}.

A VERIFIER

\begin{lemma}\label{lem:bij:iterated} 
  Let $i\in\{1,2\}$. For all $\lambda_i\in P_i$, $\reg^{G,P_i,P_{\m i}}_i(\lambda_i) =
  \reg^{G'}_i(\Phi(\lambda_i))$.
\end{lemma}

\begin{proof}
  Since there is a bijection $\Phi_H~: P_i \to \Lambda_i(H)$ we need to
  prove that there is a bijection $\Phi~: \Lambda_i(H) ŧo
  \Lambda_i(G')$.
\end{proof}




%The proof is similar to the one of Lemma~\label{lem:bij}.
%Let $(s,b_1,b_2,o_1,o_2)\in \target_i$. We define $\nu_i(s,b_1,b_2,o_1,o_2) =$

% \begin{lemma}\label{lem:maxmax:iterated}
% %   Let $i\in\{1,2\}$. For all $\lambda_i\in\Lambda_i(G')$,
% %   $\reg^{G'}_i(\lambda_i)\! =\!\!\!\!\! \max\limits_{\lambda_{\m i}\in\Lambda_{\m i}(G')}
% %   \nu_i(\lambda_1,\lambda_2)$}.

% % Moreover~:
% \vspace{-2mm}
%   $$
%   \reg^{G,H}_i = \minmax^{G'}_i
%   $$

% \vspace{-3mm}
% \end{lemma}

Thanks to the bijection of Lemma~\ref{lem:bij:iterated}, we can prove that
for all finite path $\pi$ of $G'$ leading from $s'_0$ to a state
$\last(\pi)=(s,b_1,b_2,o_1,o_2)\in S'_i$, we have $b_i=
\ba^{G,P_i,P_{\m i}}_i(\pi)$ (same proof as the proof of
Proposition~\ref{prop:ba}). Then we can prove
Proposition~\ref{lem:maxmax:iterated} in the same way we proved
Lemma~\ref{lem:maxmax} and~\ref{lemma:regretminmax}.


Let $s'=(s,b_1,b_2,o_1,o_2)\in S'$. We define $\Omega_i(s')$ as the
minimal regret value of all strategies that have at least one outcome
passing through $s'$. Formally~: we let $\Lambda_i^{G'}(s') =
\{\lambda_i \in \Lambda_i(G')\, |\, \exists \pi=\pi_0\pi_1\dots \pi_n
\dots \in \Outcome_{G'}(\lambda_i), \pi_n= s' \}$ and $\Omega_i(s') =
\min_{\lambda_i \in \Lambda_i^{G'}(s)} \reg^{G'}_i(\lambda_i)$. Since
solving \RMP on $G'$ is solving a \minmax game, we have $\Omega_i(s')=
\reg^{G'}_i (G',s')$.


The delete operator $D$ consists in removing edges $(s',s'')\in T'$
such that $s'=(s,b_1,b_2,o_1,o_2)\in S'_i$ with $o_i=\false$ and
$\Omega_i(s'') > \reg^{G'}_i$. We then remove non-rechable states to
obtain a new \DAG \twa $D(G')$.

% Figure~\ref{fig:delete:algo} gives
% the pseudo-algorithmic definition of this operator.


% \begin{figure}
% \center
% \begin{minipage}[t]{\linewidth-0.8cm}
%   {\large $D_1(G'' )$}\\[1mm]
% \begin{minipage}{8ex}{\bf Input:}\end{minipage}
%    \begin{minipage}[t]{\linewidth-1.5cm}
%     The \twa $G''$ of Definition~\ref{def:reduc:iterated}
%    \end{minipage}
% \begin{lstlisting}[style=pseudo,emph={PickAndRemove,Copy},numbers=left,numberfirstline=false]
%   Mark all states  $s''=(s,b_1,b_2,o_1,o_2)$ such that  $o_1$ is true
%   $ToDo  \leftarrow \{s''_0\}$
  
%   while $ToDo \neq\emptyset$
%      $s \leftarrow$ PickAndRemove $(ToDo)$
%      if $s\in S''_1$ then
%         for all  $(s,s')\in T''$ 
%            if $\reg_{G''}^1(s') > \reg_{G''}^1$ then
%               $T'' \leftarrow T'' \setminus \{(s,s')\}$
%            elseif $s'$ is not marked
%               $ToDo  \leftarrow Todo \cup \{s'\}$
%               Mark $s'$
%      else
%        for all  $(s,s')\in T''$   
%           if $s'$ is not marked
%              $ToDo  \leftarrow Todo \cup \{s'\}$
%              Mark $s'$
% \end{lstlisting}
% \end{minipage}
% \caption{Algorith for the Delete operator $D_1$}
% \label{fig:delete:algo}
% \end{figure}


\begin{lemma}\label{prop:correctness:iterated}
  Let $i\in\{1,2\}$. Let $\lambda_i \in \Lambda_i(G')$;
  $\reg_{G'}^i(\lambda_i) = \reg_{G'}^i$ if and only if $\lambda_i
  \in \Lambda_i(D(G'))$.
\end{lemma}

\begin{proof}
  Let $\lambda_i$ such that $\reg^{G'}_i(\lambda_i) =
  \reg^{G'}_i$. Let $\pi\in S'^*$ such as $s=\last(\pi)\in S_i'$ and
  $s'=\lambda_i(\pi)$. Since $\lambda_i\in\Lambda_i(s')$, we have
  $\Omega_i(s') \leq \reg^{G'}_i(\lambda_i)= \reg^{G'}_i$. According
  to the definition of the delete operator, $(s,s')$ is an edge of
  $D(G)$. Thus $\lambda_i\in\lambda_i(D(G'))$.

  On the other hand, if $\lambda_i \in \Lambda_i(D(G'))$. We proceed
  {\it reductio ad absurdum}.

  If $\reg^{G'}_i(\lambda_i)> \reg^{G'}_i$, there exists $\lambda_{\m
    i}\in\Lambda_{\m i}(G')$ such that
  $\reg^{G'}_i(\lambda_i,lambda_{\m i})> \reg^{G'}_i$. We let
  $\pi=\outcome(\lambda_i,\lambda_{\m i}$ and consider
  $\pi_n=(s,b_1,b_2,o_1,o_2)\in \target_i$ the first state of this
  outcome belonging to $\target_i$. Since
  $\reg^{G'}_i(\lambda_i)=\mu^{G'}_i(s)-b_i=\Omega_i(G',\pi_n)$, we
  consider the state $\pi_k\in S'_i$ such that $\pi_{k+1}\dots
  \pi_{n-1} \in (S'_{\m i})^*$. We have in $D(G')$ a transition
  $(\pi_{k},\pi_{k+1})$ such that~:
  \begin{itemize}
  \item  $\pi_{k}=(s^k,b^k_1,b^k_2,o^k_1,o^k_2)$ with $o_i=\false$
  \item $\Omega_i(\pi_{k+1})\geq \Omega_i(\pi_{n})> \reg^{G'}_i$
    because it is determined by a \minmax game with only positions of
    player $\m i$
  \item $(\pi_k,\pi_{k+1})$ is an edge of $D(G')$
  \end{itemize}
  This contradicts the definition of the operation $D(G')$. Thus
  $\reg^{G'}_i(\lambda_i) = \reg^{G'}_i$,
\end{proof}


\begin{theorem}~\ref{thm:onestep:iterated}
  Let $i\in\{1,2\}$. $\forall \lambda_i \in\Lambda_i(G)$,
  $\reg^{G,P_i,P_{\m i}}_i (\lambda_i) = \reg^{G,P_i,P_{\m i}}_i$ if
  and only if $\lambda_i \in \Phi^{-1}(\Lambda_i(D(G')))$.
\end{theorem}

\begin{proof}
  We apply the result of Lemma~\ref{prop:correctness:iterated} to the strategies of
  $G$, using the bijection of Lemma~\ref{lem:bij:iterated}.
\end{proof}


$D(G')$ thus represents the game where both players play a strategy of
$P_i$ that minimizes her regret assuming the other player plays a
strategy of $P_{\m i}$. We now show that $D(G')$ has exactly the
properties we expected from $H$:
\begin{enumerate}
\item A FAIRE
\end{enumerate}



\begin{theorem}
  Let $j>0$, $i\in\{1,2\}$ and
  $\lambda_i\in\Lambda_i(G)$. $\reg^{i,j}_G(\lambda_i)= \reg^{i,j}_G$
  if and only if $\Phi(\lambda_i) \in \Lambda_i(\widetilde{D}^j(G''))$.
\end{theorem}

\begin{proof}(sketch)
  This proof is done by induction on
  $j$. Proposition\ref{thm:onestep:iterated} ensures the
  correctness of the inductive step.
\end{proof}


By Proposition~\ref{prop:complexity:iterated} we have an upper bound
on the complexity of this computation~:

\begin{proposition}
  $\widetilde{D}^*(G'')$ may be computed in
  $O\left(|\target''_i| \times \log_{\m i}(M)\times|T''|\times(|S''|+|T''|)\right)$,
  where $M =
  \max\limits_{s\in\target_i,\mu_G^i(s)<+\infty}\mu_G^i(s)$.
\end{proposition}



==> ex2.tex <==
% Generated by Jastex 

% \documentclass{article}
% \usepackage[usenames]{color}% delete this line if you don't use colors

% \usepackage{gastex}
% \begin{document}


\begin{picture}(121,113)(0,-113)
% \put(0,-113){\framebox(121,113){}}
\node[NLangle=0.0,Nmarks=i](n0)(36.0,-32.0){$A$}

\node[NLangle=0.0](n1)(36.0,-56.0){$B$}

\node[NLangle=0.0,Nmr=0.0](n4)(36.0,-80.0){$C$}

\node[NLangle=0.0](n5)(20.0,-104.0){$D$}

\node[NLangle=0.0](n6)(52.0,-104.0){$E$}

\drawedge[ELdist=2.0](n0,n1){0}

\drawedge[ELdist=2.0](n1,n4){0}

\drawedge[ELside=r,ELdist=2.0](n4,n5){5}

\drawedge[ELdist=2.0](n4,n6){0}


\node[NLangle=0.0,Nmarks=i](n27)(95.78,-32.0){$A$}

\node[NLangle=0.0](n28)(95.78,-56.0){$B$}

\node[NLangle=0.0,Nmr=0.0](n29)(95.78,-80.0){$C$}

\node[NLangle=0.0](n30)(79.78,-104.0){$D$}

\node[NLangle=0.0](n31)(111.78,-104.0){$E$}

\drawedge[ELdist=2.0](n27,n28){0}

\drawedge[ELdist=2.0](n28,n29){0}

\drawedge[ELside=r,ELdist=2.0](n29,n30){5}

\drawedge[ELdist=2.0](n29,n31){0}

\drawedge[ELside=r,ELdist=2.0,curvedepth=-15.14](n27,n29){0}



\end{picture}
% \end{document}


==> iteratetree.tex <==
\Section{Iterated Regret Minimization}


In this section, we show how to compute the iterated
regret for weighted arenas where weights are strictly
positive. 


Let $G = (S=S_1\uplus S_2,s_0,T,\mu_G^1,\mu_G^2, \target_1, \target_2)$ 
be a weighted arena such that for all $e\in T$, $\mu_G^1(e)>0$ and
$\mu_G^2(e)>0$. Let $i\in\{1,2\}$, $S_i\subseteq \Lambda_i(G)$
and $S_{\m i}\subseteq \Lambda_{\m i}(G)$. The regret of Player $i$ when he plays 
strategies of $S_i$ and when Player $\m i$ plays strategies of $S_{\m i}$ is defined by:

$$
\begin{array}{lllllll}
\reg_{G,S_i}^i & = & \min_{\lambda_i\in S_i}\max_{\lambda_{\m i}\in S_{\m i}} \ut_G^i(\lambda_i,\lambda_{\m i}) - \br_{G,S_i}^i(\lambda_{\m i}) \text{ where } \\
\br_{G,S_i}^i(\lambda_{\m i}) & = & \min_{\lambda^*_i\in S_i} \ut_{G}^i(\lambda^*_i,\lambda_{\m i})
\end{array}
$$

let $S_i^0(G) = \Lambda_i(G)$
and for all $j>0$, $S_i^j(G)  = \{ \lambda_1\in S_i^{j-1}\ |\ \}$.


==> loopfreestrategies.tex <==
\SubSection{Loop-free strategies are sufficient to minimize the regret}

The following theorem proves that loop-free strategies are sufficient to minimize the regret
(if Player $1$ has a winning strategy).

\begin{theorem}\label{th:loopfree}
  Let $G = (S=S_1\uplus S_2,s_0,T,\mu_G^1,\target_1)$ be a weigthed game arena such that
  Player 1 has a winning strategy to reach her objective. There exists
  a loop-free Player 1's strategy $\lambda_1$ such that
  $\reg_G^1(\lambda_1) = \reg_G^1$.
\end{theorem}


\begin{proof}(Sketch)
The proof of this theorem is rather technical. It is given in Appendix.
Informally, given a winning strategy $\lambda_1\in\Lambda_1(G)$ which minimizes the regret of Player $1$,
we can see the set of outcomes as a finite tree $T_{\lambda_1}$. The nodes are partionned into Player 1's and Player 2's nodes.
The nodes carry a label from $S_1\cup S_2$ ($S_1$ for Player 1's nodes and $S_2$ for Player 2's nodes).
Let $p$ be a node of this tree.  If $p$ is labeled in $\target_1$ iff $p$ is a leaf. 
If $p$ is labelled by $s\in S_1$, then we consider the unique path from the root to reach $p$. 
The labels occuring along this path form a history $h$ of the play, and the node $p$ has
only one successor labeled $\lambda_1(h)$.
If $p$ is labeled by $s\in S_2$, we consider all possible behaviors of Player $2$, therefore
$p$ has as many successors as the successors of $s$ in $G$, which are labeled by those successors.


If there is a root-to-leave path in this tree where a label $s$ occurs twice, this label
is necessarily in $S_1$ (otherwise Player 2 would have counter-strategy to $\lambda_1$, making
Player $1$ loops infinitely). Let $p_1$ and $p_2$ be the nodes of tree where $s$ occurs, and suppose
that $p_2$ is below $p_1$. We denote by $T_{\lambda_1}'$ the tree $T_{\lambda_1}$ obtained
by replacing the subtree rooted at $p_1$ by the subtree rooted at $p_2$. This new tree
contains less nodes, and it also defines a winning strategy $\lambda_1'$ for Player $1$. We then prove
that $\lambda'_1$ also minimizes the regret of Player $1$. We can apply the same transformation
until there is no label occuring twice along a path. Thus we obtain a loop-free strategy
minmizing the regret of Player $1$.
\end{proof}

\begin{proof}(Formal Proof but old notation)
  Let $\lambda_1$ be a winning strategy that minimizes the regret and $\lambda_2$ be a strategy
  of Player 2. Let $u=\pi_1\dots\pi_n = \outcometarget(\lambda_1,\lambda_2)$, and
  suppose that there exists $i<j$ such that $\pi_i = \pi_j$. Let $h_i
  = \pi_1\dots\pi_i$, $h_j = \pi_{i+1}\dots\pi_j$. We let
  $\tilde{\lambda_1}$ be the strategy defined by:

  $$
  \tilde{\lambda_1} : h\in (S_1\cup S_2)^*S_1 \mapsto 
  \left\{\begin{array}{lllllllll}
  
  \lambda_1(h_ih_jh') & \text{ if } h = h_ih' \text{ for some $h'$} \\
  \lambda_1(h) & \text{ otherwise }
  \end{array}\right.
  $$

  We now prove three results:

  \begin{itemize}
    \item[$(i)$] $\tilde{\lambda_1}$ is winning and
      $\reg(\tilde{\lambda_1}) =  \reg(\lambda_1)$;


    \item[$(ii)$] $\outcometarget(\lambda_1) \equiv \{
  \outcometarget(\lambda_1,\lambda_2)\ |\ \lambda_2\in\Lambda_2\}$ is
  finite;

    \item[$(iii)$] $\sum\limits_{u\in\outcometarget(\tilde{\lambda_1})} |u| <
  \sum\limits_{u\in\outcometarget(\lambda_1)} |u|$.
  \end{itemize}


\vspace{2mm}
  
  \emph{Proof of $(i)$}   Let $O_{\neg i} = \{h =
  \outcometarget(\lambda_1,\lambda_2)\ |\ \lambda_2\in\Lambda_2,\ h\text{
    does not pass by } \pi_i\}$, let $O_j = \{h =
  \outcometarget(\lambda_1,\lambda_2)\ |\ \lambda_2\in\Lambda_2,\ h\text{
    passes by } \pi_j\}$. Note that all words of $O_j$ are necessarily
  of the form $h_ih_jh$, for some $h$.   By definition of $\tilde{\lambda_1}$, we
  have 
  $$
  \outcometarget(\tilde{\lambda_1}) = O_{\neg i}\cup \{
  h_ih\ |\ h_ih_jh\in O_j\}$$


  Indeed, let $\tilde{\lambda_2}\in \Lambda_2$. 
  If $\outcometarget(\tilde{\lambda_1},\tilde{\lambda_2})$ does not pass
  by $\pi_i$, and then
  $\outcometarget(\tilde{\lambda_1},\tilde{\lambda_2}) =
  \outcometarget(\lambda_1,\tilde{\lambda_2})$, and therefore
  $\outcometarget(\tilde{\lambda_1},\tilde{\lambda_2})\in O_{\neq i}$.
  If $\outcometarget(\tilde{\lambda_1},\tilde{\lambda_2})$ passes by $\pi_i$, then
  there exists some strategy $\lambda_2\in \Lambda_2$ and $h$,  such that 
  $\outcometarget(\tilde{\lambda_1},\tilde{\lambda_2}) = h_ih$ and
  $\outcometarget(\lambda_1,\lambda_2) = h_ih_jh$. 
  Intuitively, it suffices to
  take $\lambda_2$ such that it plays like $\tilde{\lambda_2}$ before
  reaching $h_i$, then play according to $h_j$ after reaching $h_i$
  and before reaching $h_ih_j$, and then play according to
  $\tilde{\lambda_2}(h_ih)$. Formally:

  $$
  \lambda_2 : h\in (S_1\cup S_2)^*S_2 \mapsto 
  \left\{\begin{array}{lllllllll}
  \tilde{\lambda_2}(h) & \text{ if } h \text{ is a prefix of $h_i$} \\
  \tilde{\lambda_2}(h_ih) & \text{ if } h=h_ih_jh' \text{ for some $h'$} \\
  \alpha & \text{ if } h=h_ih' \text{ and $h'\alpha$ is a prefix of $h_j$} \\
  \tilde{\lambda_2}(h) & \text{ otherwise}  \\
  \end{array}\right.
  $$




  Conversely, let $\lambda_2\in\Lambda_2$. If
  $\outcometarget(\lambda_1,\lambda_2)\in O_{\neg i}$, then
  $\outcometarget(\tilde{\lambda_1},\lambda_2) =
  \outcometarget(\lambda_1,\lambda_2)$. Therefore $O_{\neg i}\subseteq
  \outcometarget(\tilde{\lambda_1})$. If
  $\outcometarget(\lambda_1,\lambda_2)$ is of the form
  $h_ih_jh$, for some $h$,  there is a strategy $\tilde{\lambda_2}\in\Lambda_2$ such that
  $\outcometarget(\tilde{\lambda_1},\tilde{\lambda_2}) = h_ih$. It
  suffices to define $\tilde{\lambda_2}$ by:


  $$
  \tilde{\lambda_2} : h\in (S_1\cup S_2)^*S_2 \mapsto 
  \left\{\begin{array}{lllllllll}
  \lambda_2(h) & \text{ if } h \text{ is a prefix of $h_i$} \\
  \lambda_2(h_ih_jh') & \text{ if } h=h_ih' \text{ for some $h'$} \\
  \lambda_2(h) & \text{ otherwise}  \\
  \end{array}\right.
  $$
  


  We now prove that $\reg(\tilde{\lambda_1})\leq \reg(\lambda_1)$, and
  therefore $\reg(\tilde{\lambda_1}) = \reg(\lambda_1)$ since
  $\lambda_1$ minimizes the regret in $G$. Let $\tilde{\lambda_2}$
  which maximizes $\reg(\tilde{\lambda_1})$. Let $o =
  \outcometarget(\tilde{\lambda_1},\tilde{\lambda_2})$.
  If $h_i$ is not a prefix of $o$, then   $o =
  \outcometarget(\lambda_1,\tilde{\lambda_2})$, and therefore 
  $\reg(\tilde{\lambda_1},\tilde{\lambda_2}) =
  \reg(\lambda_1,\tilde{\lambda_2}) \leq \reg(\lambda_1)$. If $o =
  h_ih$, for some $h$, then we consider the following strategy
  $\lambda_2$:


  $$
  \lambda_2 : h\in (S_1\cup S_2)^*S_2 \mapsto 
  \left\{\begin{array}{lllllllll}
  \alpha & \text{ if $h\alpha$ is a prefix of $h_ih_j$} \\
  \tilde{\lambda_2}(h_ih') & \text{ if } h=h_ih_jh' \text{ for some $h'$} \\
  \tilde{\lambda_2}(h) & \text{ otherwise}  \\
  \end{array}\right.
  $$


  \emph{Claim.} $\br(\lambda_2)\leq \br(\tilde{\lambda_2}) + u(h_j)$.

  \begin{proof}
   
    Let $\lambda_1^*$ be a best response to
    $\tilde{\lambda_2}$. We consider two cases:

    \begin{itemize}
      \item if $h_i$ is not a prefix of
        $\outcometarget(\lambda_1^*,\tilde{\lambda_2})$, then 
        $\outcometarget(\lambda_1^*,\tilde{\lambda_2}) =
        \outcometarget(\lambda_1^*,\lambda_2)$. Therefore 
        $u(\lambda_1^*,\lambda_2) = u(\lambda_1^*,\tilde{\lambda_2}) =
        \br(\tilde{\lambda_2})$, and clearly, $\br(\lambda_2)\leq
        u(\lambda_1^*,\lambda_2) = \br(\tilde{\lambda_2})\leq
        \br(\tilde{\lambda_2}) + u(h_i)$;

      \item if $\outcometarget(\lambda_1^*,\tilde{\lambda_2}) = h_ih'$
        for some $h'$, we construct some strategy $\hat{\lambda_1}$ such
        that $u(\hat{\lambda_1},\lambda_2) =
        u(\lambda_1^*,\tilde{\lambda_2}) + u(h_j)$. This strategy
        is defined by:

        $$
        \hat{\lambda_1} : h\in (S_1\cup S_2)^*S_1 \mapsto 
        \left\{\begin{array}{lllllllll}
        \alpha & \text{ if $h\alpha$ is a prefix of $h_ih_j$} \\
        \lambda_1^*(h_ih') & \text{ if } h=h_ih_jh' \text{ for some $h'$} \\
        \lambda_1^*(h) & \text{ otherwise}  \\
        \end{array}\right.
        $$

        We know that $\outcometarget(\lambda_1^*,\tilde{\lambda_2}) =
        h_ih'$. By definition of $\hat{\lambda_1}$,
        $\outcometarget(\hat{\lambda_1},\tilde{\lambda_2})$ is
        necessarily of the form $h_ih''$, for some $h''$. Suppose that
        $\pi_i\in S_1$. By definition of $\hat{\lambda_1}$,
        $\hat{\lambda_1}(h_i) = \pi_{i+1}$. If $\pi_{i+1}\in S_2$, by definition of
        $\lambda_2$, $\lambda_2(h_i\pi_{i+1}) = \pi_{i+2}$.  
        More generally, by some induction argument, we can prove $\outcometarget(\hat{\lambda_1},\lambda_2) =
        h_ih_jh'''$, for some $h'''$. If $\pi_j\in S_1$, then by
        definition of $\hat{\lambda_1}$, $\hat{\lambda_1}(h_ih_j) =
        \lambda_1^*(h_i)$. Let $\pi_{j+1} = \lambda_1^*$. If
        $\pi_{j+1}\in S_2$, then by definition of $\lambda_2$,
        $\lambda_2(h_ih_j\pi_{j+1}) =
        \tilde{\lambda_2}(h_i\pi_{j+1})$. Let $\pi_{j+2} =
        \lambda_2(h_ih_j\pi_{j+1})$. If $\pi_{j+2}\in S_1$, then 
        $\hat{\lambda_1}(h_ih_j\pi_{j+1}\pi_{j+2})
        =
        \tilde{\lambda_1}(h_i\pi_{j+1}\pi_{j+2})$. More generally, by
        some induction argument, we can prove that
        $\outcometarget(\lambda_1^*,\tilde{\lambda_2}) = h_ih'''$. 
        Therefore $\br(\tilde{\lambda_2}) = u(\lambda_1^*,\tilde{\lambda_2}) =
        u(\hat{\lambda_1},\lambda_2) - u(h_j)\geq \br(\lambda_2)-u(h_j)$. 
    \end{itemize}
 
  $\hfill$\emph{End of Claim Proof}\end{proof}


  We have $u(\lambda_1,\lambda_2) =
  u(\tilde{\lambda_1},\tilde{\lambda_2}) + u(h_j)$. By the claim, we
  get $u(\lambda_1,\lambda_2) - \br(\lambda_2) \geq 
  u(\tilde{\lambda_1},\tilde{\lambda_2}) - \br(\tilde{\lambda_2}) = \reg(\tilde{\lambda_1})$,
  and therefore $\reg(\lambda_1)\geq \reg(\tilde{\lambda_1})$.



\vspace{2mm}
  
  

  \emph{Proof of $(ii)$}
  We can see the set $\outcometarget(\lambda_1)$ as a
  tree $T_{\lambda_1} = (V, E)$ where
  $V = pref(\outcometarget(\lambda_1))$ is the set of prefixes of
  $\outcometarget(\lambda_1)$, and $E$ is defined by $\forall u\in
  V$, for all $a\in S_1\cup S_2$, $(u,ua)\in E$ if there exists
  $\lambda_2$ such that $u$ and $ua$ are prefixes of
  $\outcometarget(\lambda_1,\lambda_2)$. Note that $a = \lambda_1(u)$
  if $\last(u)\in S_1$, and $a$ ranges over 
  $\{ s\ |\ (\last(u),s)\in T\}$ otherwise. Therefore $T_{\lambda_1}$ is finite
  branching. Therefore if $\outcometarget(\lambda_1)$ is infinite, by
  König's Lemma, there is an infinite path $\pi = \pi_1\pi_2\dots$ in
  $T$. Therefore Player 1 cannot reach the objective against the
  strategy $\lambda_2$ defined by $\lambda_2(\pi_1\dots\pi_i) =
  \pi_{i+1}$ for all $i$ such that $\pi_i\in S_2$, which contradicts
  the fact that $\lambda_1$ is winning.




\vspace{2mm}


  \emph{Proof of $(iii)$}
  Let $O_{\neg i}$ and $O_j$ be defined as for item $(i)$.
  We have $\sum_{u\in O_{\neg i}} |u| + \sum_{u\in\{h_ih\ |\ h_ih_jh} |u| =
  \sum_{u\in O_{\neg i}} |u| + \sum_{u\in O_j} (|u| - |h_j|)$, and
  since $|h_j|>0$, we get $\sum_{u\in O_{\neg i}} |u| + \sum_{u\in
    O_j} (|u| - |h_j|) < \sum_{u\in O_{\neg i}} |u| + \sum_{u\in
    O_j} |u| \leq \sum_{u\in\outcometarget(\lambda_1)} |u|$. 





\vspace{2mm}


  As a conclusion, items $(i)$, $(ii)$ and $(iii)$ give a way to
  construct a loop-free strategy $\lambda_1'$ such that $\reg(\lambda_1') =
  \reg(\lambda_1) = \reg(G)$ by iterating the construction 
  used to define $\tilde{\lambda_1}$. It terminates since the quantity in item
  $(iii)$ strictly decreases and is bounded by $0$.
\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> trees.tex <==
\Section{Regret Minimization in Finite Trees}\label{sec:trees}

In this section, we consider target-weighted tree arenas, on which the regret
minimization problem can be defined similarly as for weighted tree
arenas. In particular, the notion of best response carries over to
target-weighted arenas. The \RMP on tree arenas can be easily reduced
to
the \RMP on target-weighted arenas, since target nodes are reachable
by a unique path from the initial position. Therefore the value of
target node in the target-weighted arena will be the value of the
unique path to reach it in the weighted arena. Moreove, since both
players play symmectric roles, wlog we can suppose that we want
to compute the regret of Player $1$, and omit the target and weight
function of Player $2$.



Let $G = (S=S_1\uplus S_2,s_0,T,\mu_G^1,\target_1)$ be a target-weighted
tree arena. Let $s\in S_1$. The best value that can be achieved from
node $s$ by Player $1$ when Player 2 cooperates is defined by:

$$
\best_G^1(s) = \min_{\lambda_1\in \Lambda_1(G,s)}
\min_{\lambda_2\in\Lambda_2(G,s)} \ut_G^1(\lambda_1,\lambda_2)
$$


Let now $(s,s')\in T$. The \textit{best
  alternative} of choosing $s'$ from $s$ for Player $1$, denoted by $\ba^G_1(s,s')$, 
is defined as the minimal value he could have achieved if he were able
to choose another successor of $s$. Formally:

$$
\ba_G^1(s,s') = \left\{\begin{array}{lllll}
+\infty & \text{ if } s\in S_{2} \\
\min_{(s,s'')\in T,s''\neq s'} \best_G^1(s) & \text{ if } s\in S_{1} \\
\end{array}\right.
$$

Finally, the best alternative of a path $\pi = s_0s_1\dots s_n$ is
defined as $+\infty$ if $n=0$ and as the minimal
best alternative of the edges of $\pi$ otherwise:

$$
\ba_G^1(\pi) = \min_{0\leq j<n} \ba^1_G(s_j,s_{j+1})
$$

Let $s\in S$. There is a unique path $\pi$ from the root to $s$,
therefore we can define the best alternative of $s$ as 
$\ba_G^1(s) = \ba_G^1(\pi)$. 


Informally, let $\lambda_1\in\Lambda_1(G)$ and
$\lambda_2\in\Lambda_2(G)$ which maximizes
$\reg_G^1(\lambda_1,\lambda_2)$. If $\lambda_1$ is winning, then
$\outcome_G^1(\lambda_1,\lambda_2)$ contains Player 1's target positions.
Let $s$ be the first target position occuring in
$\outcome_G^1(\lambda_1,\lambda_2)$. To
maximize $\reg_1(\lambda_1,\lambda_2)$, Player 2 may cooperate
with Player 1 in the subtrees where Player 1 did not choose to go.  This cooperation
is represented by the best alternative. It is formally states in the
next lemma:


\begin{lemma}\label{lem:tree}
  Let $\lambda_1\in\Lambda_1(G)$ and $\lambda_2\in\Lambda_2(G)$ which
  maximizes $\reg_G^1(\lambda_1,\lambda_2)$. If $\lambda_1$ is winning, then 
  $$
  \reg_G^1(\lambda_1,\lambda_2) =
  \mu_G^1(s)-\min(\mu_G^1(s),\ba_G^1(s))
  $$
  where $s\in\target_1$ is the first occurence of a target node 
  in $\outcome_G(\lambda_1,\lambda_2)$.  \end{lemma}

\begin{proof}
  Let $\pi = s_0s_1\dots s_n$ be a prefix of
  $\outcome_G(\lambda_1,\lambda_2)$ such that $s_n = s$ is the first
  occurence of a target node. We define a strategy $\lambda'_2$ that
  plays as $\lambda_2$ along $\pi$ and cooperate with Player $1$ in the
  subtrees that Player $1$ did not choose. Formally, for all $h\in
  \play(G)$ such that $\last(h)\in S_2$, we let 
  $\lambda'_2(h) = s_{j+1}$ if there is $j<n$ such that $h =
  s_0s_1\dots s_j$. Otherwise we let 
  $\lambda'_2(h) = s'$ where $s'$ minimizes $\best(s'')$, for all
  $s''$ such that $(\last(h),s'')\in T$.Formally, for all $h\in
  \play(G)$ such that $\last(h)\in S_2$, we let 
  $\lambda'_2(h) = s_{j+1}$ if there is $j<n$ such that $h =
  s_0s_1\dots s_j$. Otherwise we let 
  $\lambda'_2(h) = s'$ where $s'$ minimizes $\best(s'')$, for all
  $s''$ such that $(\last(h),s'')\in T$. Clearly,
  $\outcome_G^1(\lambda_1,\lambda_2) =
  \outcome_G^1(\lambda_1,\lambda'_2)$. Since $\lambda'_2$ minimizes
  the utility in subtrees where the strategy $\lambda_1$ prevents to
  go, we have $\br_G^1(\lambda'_2)\leq \br_G^1(\lambda_2)$. Since
  $\lambda_2$ maximizes $\reg_G^1(\lambda_1,\lambda_2)$, we get
  $\reg_G^1(\lambda_1,\lambda_2) = \reg_G^1(\lambda_1,\lambda'_2)$.
  The best response to
  $\lambda_2$ either deviates from $\pi$ or not. In particular, if the
  best response chooses to deviate from $\pi$ at a node $s_j$ $j<n$,
  i.e. chooses a node $s'$ such that $s'\neq s_j$, then the utility 
  of the best response, according to the definition of $\lambda'_2$,
  is $\best_G^1(s')$. The best response should minimize over all those
  possibilities, therefore $\reg_G^1(\lambda_1,\lambda'_2) = \mu_G^1(s)
  - \min(\mu_G^1(s),\min_{j<n,(s_j,s')\in T, s'\neq s_{j+1}}
  \best(s'))$, i.e. $\mu_G^1(s)-\min(\mu_G^1(s),\ba_G^1(s))$.
 \end{proof}


\begin{lemma}\label{lem:treeback}
  Let $\lambda_1\in\Lambda_1(G)$ and $\lambda_2\in\Lambda_2(G)$. 
  If $\lambda_1$ is winning, then there exists $\lambda_2'\in\Lambda_2(G)$ such that
  
  $$
  \reg_G^1(\lambda_1,\lambda'_2) =
  \mu_G^1(s)-\min(\mu_G^1(s),\ba_G^1(s))
  $$
  where $s\in\target_1$ is the first occurence of a target node 
  in $\outcome_G(\lambda_1,\lambda_2)$.
\end{lemma}

\begin{proof}
  The construction of $\lambda_2'$ is similar to the proof of Lemma \ref{lem:tree}. Informally, $\lambda'_2$ plays
  as $\lambda_2$ on the path $\outcome_G(\lambda_1,\lambda_2)$ and
  cooperate (i.e. minimizes the utility) in subtrees where the
  strategy $\lambda_1$ prevents to go. 
\end{proof}

We can now reduce the \RMP to a \minmax game:

\begin{lemma}
  Let $G = (S,s_0,T,\mu_G^1,\target_1)$ and let $\mu_{G'}^1 :
  s\in\target_1\mapsto \mu_G^1(s) - \min(\mu_G^1(s),\ba_G^1(s))$.
  Let $G' = (S,s_0,T,\mu_{G'}^1,\target_1)$. Then $\reg_G^1 =
  \minmax_{G'}^1$.
\end{lemma}


\begin{proof}
  First note that $\Lambda_i(G) = \Lambda_i(G')$ for all $i\in\{1,2\}$
  and a Player 1's strategy is winning in $G$ iff it is winning
  in $G'$.  Therefore $\reg_G^1<+\infty$ iff
  $\minmax_{G'}^1<+\infty$. Let $W_1(G)$ be the set of winning
  strategies of Player 1 in $G$, and suppose that
  $W_1(G)\neq\varnothing$. Let $\lambda_1\in W_1(G)$. We have
  $\max_{\lambda_2\in \Lambda_2(G')} \ut_{G'}^1(\lambda_1,\lambda_2) =
  \max_{\lambda_2\in \Lambda_2(G)} \reg_G^1(\lambda_1,\lambda_2)$. Indeed, the
  inequality $\geq$ is a consequence of Lemma \ref{lem:tree}, while the inequality $\leq$ is a consequence of Lemma \ref{lem:treeback}.
  Therefore we get:
  $$
  \begin{array}{lllllll}
  & & \min_{\lambda_1\in\Lambda_1(G)}  & \max_{\lambda_2\in\Lambda_2(G)}
  & \reg_G^1(\lambda_1,\lambda_2) \\
  & = &   \min_{\lambda_1\in W_1(G)}&  \max_{\lambda_2\in\Lambda_2(G)}
  & \reg_G^1(\lambda_1,\lambda_2) \\
  & = & \min_{\lambda_1\in W_1(G')} & \max_{\lambda_2\in\Lambda_2(G')}
  & \ut_{G'}^1(\lambda_1,\lambda_2) \\
  & = & \min_{\lambda_1\in \Lambda_1(G')} & \max_{\lambda_2\in\Lambda_2(G')}
  & \ut_{G'}^1(\lambda_1,\lambda_2) \\
  \end{array}
  $$
\end{proof}


The \textit{size} of a target-weighted tree arena $G = (S,s_0,T,\mu_G^1,\mu_G^2,\target_1,\target_2)$ is defined by
$\size{G} = |S|+\sum_{s\in\target_1} log_2(\mu_G^1(s)) +
\sum_{s\in\target_2} log_2(\mu_G^2(s))$. 


\begin{theorem}
  The \RMP on a target-weighted tree arena $G =
  (S,s_0,T,\mu_G^1,\mu_G^2,\target_1, \target_2)$ can be solved in time 
  $O(\size{G}.log M)$, where $M = \max_{s\in\target_1}\mu_G^1(s)$.
\end{theorem}

\begin{proof}
  Suppose that we want to compute $\reg_G^1$. In a first step, we
  compute the values $\best(s)$ for all $s\in \target_1$. This can be
  done in time $O(\size{G})$ by a one-pass bottom-up algorithm which keeps, for all inner node, the 
  minimal value of the values computed for its children. Let $s\in S$ and $s_1,\dots,s_n$ its children, ordered such that
  $\best(s_1)\leq \dots \best(s_n)$. If $n = 1$, then $\ba(s,s_1)=+\infty$. Otherwise for all $j\neq 1$, we have $\ba(s,s_j) = \ba(s,s_1)$ if $j\neq 1$, and
  $\ba(s,s_1)=\ba(s,s_2)$. Therefore we can compute the values $\ba(s,s')$ for all edges $(s,s')\in T$ in time $O(\size{G})$. Computing the values
  $\ba(s)$, for all $s\in\target_1$ can finally be done in time $O(\size{G})$ by a one-pass top-down algorithm which keeps, for all $s\in S$, the minimal best alternative
  seen so far along the unique path from $s_0$ to $s$. Finally, it remains to solve a $\minmax$ game, which can be done in $O(log_2(M')|S|)$ (Prop \ref{prop:minmaxgame}), where
  $M' = \max_{s\in C_1} (\mu_G^1(s) - \min(\mu_G^1(s),\ba_G^1(s))) \leq M$.
\end{proof}

